Parametrization of PSL(2,C)-representations of surface groups

For an oriented surface of genus g with b boundary components, we construct a rational map from a subset of C^{6g-6+3b} onto an open algebraic subset of the PSL(2,C)-character variety as an analogue of the Fenchel-Nielsen coordinates. After taking the quotient by an action of a finite group, we obtain a parametrization of a subset of the PSL(2,C)-character variety, and similarly for the SL(2,C)-character variety. We can systematically calculate a set of matrix generators by rational functions of the parameters. We give transformation formulae under elementary moves of pants decompositions.

==> sec_euler_class.tex <==
%
% want to add this sebsection to sec_pslr.tex
%
\subsection{Euler class}
We study other real components.
First of all, we recall the Euler class of a $\PSLR$-representation.

Let $\widetilde{\mathrm{PSL}(2,\mathbb{R})}$ be the universal covering of $\PSLR$.
We say that an element of $\widetilde{\mathrm{PSL}(2,\mathbb{R})}$ is hyperbolic (resp. parabolic, elliptic) if it is mapped to a hyperbolic (resp. parabolic, elliptic) 
element in $\PSLR$.
Let $\widetilde{\exp} : \mathfrak{g} \to \widetilde{\mathrm{PSL}(2,\mathbb{R})}$ be the exponential map.
The center of $\widetilde{\PSLR}$ is
 \[
\left\{ \widetilde{\exp} ( \begin{pmatrix} 0 & -n\pi \\ n\pi & 0 \end{pmatrix}) \mid n \in \mathbb{Z} \right\}.
\]
We let $\mathrm{Hyp}_0$ be the set of hyperbolic elements which lie on one-parameter subgroups.
% We define $\mathrm{Hyp}_n = \widetilde{\exp} ( \begin{pmatrix} 0 & -n\pi \\ n\pi & 0 \end{pmatrix} ) \cdot \mathrm{Hyp}_0$.
Any hyperbolic element of $\widetilde{\mathrm{PSL}(2,\mathbb{R})}$ is contained in 
$\mathrm{Hyp}_n = \widetilde{\exp} ( \begin{pmatrix} 0 & -n\pi \\ n\pi & 0 \end{pmatrix} ) \mathrm{Hyp}_0$ for some $n$.

Let $S$ be a compact oriented surface.
There is a presentation of $\pi_1(S)$ as 
\[
\langle \alpha_1, \dots, \alpha_g, \beta_1, \dots, \beta_g, \delta_1, \dots, \delta_b  \mid [\alpha_1,\beta_1] \dots [\alpha_g,\beta_g] \delta_1 \dots \delta_b = 1 \rangle
\]
Let $\rho:\pi_1(S) \to \PSLR$ be a representation such that $\rho(\delta_i)$ are hyperbolic.
We see that $\rho(\delta_i)$ has a unique $\widetilde{C}_i$ lift in $\mathrm{Hyp}_0$.
We take a lift $\widetilde{A}_i$ (resp. $\widetilde{B}_i$) of $\rho(\alpha_i)$ (resp. $\beta_i$) in $\widetilde{\PSLR}$.
Then 
\[
[\widetilde{A}_1,\widetilde{B}_1] \dots [\widetilde{A}_g,\widetilde{B}_g] \widetilde{C}_1 \dots \widetilde{C}_b 
\]
is in the center of $\widetilde{\PSLR}$.
Therefore equal to $\begin{pmatrix} 0 & -n\pi \\ n\pi & 0 \end{pmatrix}$ for some $n$.
The relative Euler class $e(\rho)$ is equal to $n [S]$ where $[S] \in H^2(S, \partial S; \mathbb{Z})$ is the fundamental class of $S$.  

\begin{figure}
\input{sl2r.pstex_t}
\caption{The structure of $\widetilde{\PSLR}$.}
\label{fig:sl2r}
\end{figure}

\begin{proposition}[Additivity]
Suppose that $S= S_1 \cup S_2$ and $\rho$ has the property.
Then we have
\[
e(\rho) = e(\rho|_{\pi_1(S_1)}) + e(\rho|_{\pi_1(S_2)} )
\]
\end{proposition}

\begin{proposition}[\cite{goldman}]
Let $S$ be a pair of pants or a one-holed torus.
Suppose that $\rho$ satisfies the property.
Then $e(\rho)$ is $-1$, $0$ or $+1$.
$\rho$ is discrete faithful if and only if $e(\rho) = \pm 1$.
\end{proposition}






\begin{proposition}
$e(\rho)$ is equal to the number of positively oriented ideal triangles minus negatively oriented ideal triangles.
\end{proposition}


